Uncertainty Quantification of Collaborative Detection for Self-Driving

Sharing information between connected and autonomous vehicles (CAVs) fundamentally improves the performance of collaborative object detection for self-driving. However, CAVs still have uncertainties on object detection due to practical challenges, which will affect the later modules in self-driving such as planning and control. Hence, uncertainty quantification is crucial for safety-critical systems such as CAVs. Our work is the first to estimate the uncertainty of collaborative object detection. We propose a novel uncertainty quantification method, called Double-M Quantification, which tailors a moving block bootstrap (MBB) algorithm with direct modeling of the multivariant Gaussian distribution of each corner of the bounding box. Our method captures both the epistemic uncertainty and aleatoric uncertainty with one inference pass based on the offline Double-M training process. And it can be used with different collaborative object detectors. Through experiments on the comprehensive collaborative perception dataset, we show that our Double-M method achieves more than 4X improvement on uncertainty score and more than 3% accuracy improvement, compared with the state-of-the-art uncertainty quantification methods. Our code is public on https://coperception.github.io/double-m-quantification.

==> coperception.tex <==
\section{Collaborative 3D Object Detection}\label{sec:collab}
The agent $i$ $(i=0,1,\ldots,N)$ uses a LiDAR to create a local binary bird's eye view (BEV) map $\mathbf{M}_{i} \in \{0, 1\}^{W \times L \times H}$, where $N$ is the number of agents, and $W$, $L$, and $H$ indicate the width, length, and height of the local BEV map respectively. We consider homogeneous collaborative detection, in which multiple agents share the same detector which consists of an encoder denoted by $\theta$, and an aggregator as well as a decoder that are collectively represented by $\psi$. $\theta$ compresses the BEV map into an intermediate feature map $\mathbf{F}_i\in \mathbb{R}^{\frac{W}{K} \times \frac{L}{K} \times C} = \theta(\mathbf{M}_{i})$, where $K$ is the spatial downsampling scale, and $C$ is the feature dimension. Afterwards, $\mathbf{F}_i$ is sent to other agents, and the agent $i$ will use $\psi$ to generate a set of bounding boxes $\hat{\mathbf{Y}}_s = \psi(\mathbf{F}_i, \{ \mathbf{F}_j \}_{j \neq i})$. During training, $\theta$ and $\psi$ are jointly learned by minimizing the detection loss $\mathcal{L}_{det}(\hat{\mathbf{Y}}_s, \mathbf{Y}_{gt})$, where $\mathbf{Y}_{gt}$ denotes ground-truth boxes. $\mathcal{L}_{det}$ includes a classification loss and a regression loss following existing detectors~\cite{luo2018fast}.

==> old_approach.tex <==
\section{Uncertainty Quantification Approach}
\label{sec:approach}
%\comment{How to write the approach part to show that our uncertainty quantification method is designed for collaborative Object Detection. We want to emphasize that our methodology has novelty, not just apply one method on collaborative obejct detection? Keypoints: 1. mbb and dm are not relay on special neural network structure 2. direct modeling only add one head on the final part and change the loss function (explain the reason why we choose this loss function) 3. mbb is good on the tempor dataset 3. Our method is suitable for different models of collaborative perception design, not only for one specific model (by MBB+direct modeling). 5.In terms loss function design, we want to emphasize that: we select four vertex coordinate, consider each vertex independent and direct model a 2 by 2 covariance matrix for each vertex, this representation of uncertainty set is designed according to CAV multi-view ; and, the loss function considers both accuracy and covariance, to make sure that the trained model cares about both accuracy rate and uncertainty: the loss function improves accurate rate and also punishes over confident prediction. Both accuracy and uncertainty quantification are important for multi-view object detection}

In this section, we first introduce the problem description. Then we propose our design on direct modeling with loss function. Finally, we propose our novel \mdm \  method.  One major novelty of our algorithm is the first MBB-based algorithm to address the uncertainty quantification challenge of collaborative object detection, and the sample-based epistemic uncertainty is estimated through offline training with no inference needed. The algorithm does not rely on a specific neural network model or structure and can be used with different collaborative object detectors. Meanwhile, our design does not need to modify the neural network model structure of a collaborative object detector (such as DiscoNet~\cite{li2022v2x}) and estimates the aleatoric uncertainty with one inference in addition to the MBB process. We also design the corresponding loss function with both the prediction accuracy and covariance as metrics. 

\begin{figure*}[t]
    \centering    
    \includegraphics[width=0.99\textwidth]{figure/main.pdf}
    \vspace{-1mm}
    \caption{Probabilistic collaborative object detection. \textbf{(a) Early collaboration} shares raw point cloud with other agents, and \textbf{(b) intermediate collaboration} shares intermediate feature representations with other agents. We use direct modeling to predict the covariance matrix $\hat{\Sigma}$ and then combine it with $\Sigma_e$ and $\Sigma_a$ from MBB  as the estimated covariance matrix $\bar{\Sigma}$.   }
    \label{fig:main}
    \vspace{-3mm}
\end{figure*}

\subsection{Problem Description}

We use $X$ to represent the point cloud data. For the deterministic collaborative Object detection, the agent $\alpha \in \{1,\ldots,N \}$ create a local binary~\ac{bev} map $\mathcal{M} \in \{0, 1\}^{W_m \times L_m \times H_m}$ from $X$, where $N$ is the number of agents, and $W_m$, $L_m$, and $H_m$ indicate the width, length, and height of the local~\ac{bev} map respectively~\cite{wu2020motionnet}. As shown in Figure~\ref{fig:main} (a), we consider homogeneous collaborative object detection, in which multiple agents share the same detector $f_\theta$ which consists of an encoder denoted by $\mathcal{E}$, and an aggregator as well as a decoder that is collectively represented by $\mathcal{D}$, where $\theta$ denotes the parameters of $f$. $\mathcal{E}$ compresses the~\ac{bev} map into an intermediate feature map $\mathbf{F}_\alpha \in \mathbb{R}^{\frac{W_m}{K_m} \times \frac{L_m}{K_m} \times F_m} = \mathcal{E}(\mathcal{M})$, where $K_m$ is the spatial downsampling scale, and $F_m$ is the feature dimension. Afterwards, $\mathbf{F}_\alpha$ is sent to other agents, and the agent $\alpha$ will use $\mathcal{D}$ to generate a set of bounding boxes $\hat{Y} = \mathcal{D}(\mathbf{F}_\alpha, \{ \mathbf{F}_\beta \}_{\beta \neq \alpha})$. During training, $\mathcal{E}$ and $\mathcal{D}$ are jointly learned by minimizing the detection loss $\mathcal{L}_{det}(Y, \hat{Y})$, where $Y$ denotes the set of ground-truth boxes. $\mathcal{L}_{det}$ includes a classification loss and a regression loss. Note that we also consider early collaboration which shares raw point cloud as shown in Figure~\ref{fig:main} (b), we omit its notations for simplicity because the only thing that sets it apart from intermediate collaboration is the timing of information sharing.

%Each bounding box contains the class and $I$ corners. \songyang{Each bounding box contains $I$ corners.} Each corner $i \in \{1, \ldots, I\}$ is represented by a $D$-dimensional vector in the~\ac{bev} map. The ground-truth bounding box in $Y$ is defined as $ y = \{ c, \{y_{1},y_{2},...,y_{I}\} \}$ where $c$ is the classification label and $y_{i} \in \mathbb{R}^D (\forall i = 1, ..., I)$. The predicted bounding box in $\hat{Y}$ is defined as $\hat{y} = \{ \hat{p}, \{\hat{y}_{1},\hat{y}_{2},...,\hat{y}_{I}\} \}$, where $\hat{p}$ is the predicted classification probability and $\hat{y}_{i} \in \mathbb{R}^D ( \forall i = 1, ..., I)$ \songyang{is the predicted coordinate of corner $i$}. For the probabilistic object detection, we predict the distribution of each corner $i$ with $\hat{y}_i$ as the mean and $\hat{\Sigma}_{i}$ as the covariance. The $D \times D$ covariance matrix $\hat{\Sigma}_i$ quantifies the uncertainty of $i$-th corner.  So $\hat{y}$ is changed to $\{ \hat{p},  \{\hat{y}_i, \hat{\Sigma}_i\}_{i=1}^I \}$.

In each point cloud data $X$, there are $J$ objects. For each object $j \in \{1, \ldots, J \}$, we propose to predict $I$ corners of the bounding box. Each corner $i \in \{1, \ldots, I\}$ is represented by a $D$-dimensional vector in the~\ac{bev} map. The set of ground-truth bounding boxes $Y$ is represented as $ Y = \{ c_j, \{y_{ij}\}_{i=1}^I \}_{j=1}^J$ where $c$ is the classification label and $y_{ij} \in \mathbb{R}^D (\forall i = 1, ..., I, \forall j = 1, ..., J)$. The set of predicted bounding box $\hat{Y}$ is represented as $\hat{Y} = \{ \hat{p}_j,  \{\hat{y}_{ij}, \hat{\Sigma}_{ij}\}_{i=1}^I \}_{j=1}^J $, where $\hat{p}$ is the predicted classification probability and $\hat{y}_{ij} \in \mathbb{R}^D ( \forall i = 1, ..., I, \forall j = 1, ..., J)$ is the predicted coordinate of corner $i$ of object $j$, $\hat{\Sigma}_{ij}$ is a $D \times D$ covariance matrix. 

% For one object detection dataset, we consider $K$ frames. For frame $k \in \{1, \ldots, K\}$, there are $J$ objects. When we train or test the detector with this dataset, for $k$-th frame, we have the point cloud data $X_k$ and the ground-truth $Y_k = \{ 
% \{ c_{jk}, \{y_{ijk}\}_{i=1}^I  \}_{j=1}^J \}$. With input $X_k$, the output from the probabilistic object detector $f_{\theta}$ is:
% \begin{equation}
%     f_{\theta}(X_k) = \hat{Y}_k = \{ \{\hat{p}_{jk}, \{\hat{y}_{ijk}, \hat{\Sigma}_{ijk} \}_{i=1}^I \}_{j=1}^J \}, \label{eq:dm-output}
% \end{equation}
% where $\theta$ represents parameters of the object detector, $\hat{p}_{jk}$ is the predicted classification possibility for the $j$-th object in the $k$-th frame, $\hat{y}_{ijk}$ and $\hat{\Sigma}_{ijk}$ are the predicted mean vector and covariance matrix for the $i$-th corner of the $j$-th object in the $k$-th frame.

Finally, we model all corners are independent, and the distribution of each corner is a multivariate Gaussian distribution with parameters $\hat{y}_{ij}$ and $\bar{\Sigma}_{ij}$, where $\bar{\Sigma}_{ij}=\Sigma_{e} + (\frac{1}{2}\Sigma_{a} + \frac{1}{2}\hat{\Sigma}_{ij})$.
In the following subsection~\ref{sec:direct_modeling}, we introduce the loss function of the object detector. Then in subsection~\ref{sec:doubleM}, we propose our novel design, the main contribution of this work, the Double-M Quantification algorithm to train the object detector and learn $\Sigma_a$ and $\Sigma_e$.

%The agent $\alpha \in \{1,\ldots,N \}$ uses a LiDAR to create a local binary~\ac{bev} map $\mathbf{M}_{\alpha} \in \{0, 1\}^{W_m \times L_m \times H_m}$, where $N$ is the number of agents, and $W_m$, $L_m$, and $H_m$ indicate the width, length, and height of the local~\ac{bev} map respectively~\cite{wu2020motionnet}. As shown in Figure~\ref{fig:main}, we consider homogeneous collaborative detection, in which multiple agents share the same detector which consists of an encoder denoted by $\mathcal{E}$, and an aggregator as well as a decoder that are collectively represented by $\mathcal{D}$. $\mathcal{E}$ compresses the~\ac{bev} map into an intermediate feature map $\mathbf{F}_a\in \mathbb{R}^{\frac{W_m}{K_m} \times \frac{L_m}{K_m} \times F_m} = \mathcal{E}(\mathbf{M}_{a})$, where $K_m$ is the spatial downsampling scale, and $F_m$ is the feature dimension. Afterwards, $\mathbf{F}_a$ is sent to other agents, and the agent $a$ will use $\mathcal{D}$ to generate a set of bounding boxes $\hat{Y} = \mathcal{D}(\mathbf{F}_\alpha, \{ \mathbf{F}_\beta \}_{\beta \neq \alpha})$. During training, $\mathcal{E}$ and $\mathcal{D}$ are jointly learned by minimizing the detection loss $\mathcal{L}(\hat{Y}, Y)$, where $Y$ denotes ground-truth boxes. $\mathcal{L}$ includes a classification loss and a regression loss following existing detectors~\cite{luo2018fast}.

%We use~\ac{bev} map to represent the map, which is a widely used and powerful representation in autonomous driving~\cite{wu2020motionnet}. Given the voxelized point cloud, the collaborative object detectors recognize and localize the objects with~\ac{bev} bounding box.
%\songyang{We consider $K$ frames. For frame $k \in \{1, \ldots, K\}$, there are $J$ objects. For each object $j \in \{1, \ldots, J \}$, we propose to predict $I$ corners of the bounding box.} Each corner $i \in \{1, \ldots, I\}$ is represented by one $D$-dimensional vector in the~\ac{bev} map. Here we use $\hat{y} = \{\hat{y}_{1},\hat{y}_{2},...,\hat{y}_{I}\} \ (\hat{y}_{i} \in \mathbb{R}^D, \forall i = 1, ..., I)$ to represent the predicted bounding box, and $\hat{p} \in \mathbb{R}^C$ is the predicted classification probability for the $C$ classes. The ground-truth bounding box is defined as $ y = \{y_{1},y_{2},...,y_{I} \}\ (y_{i} \in \mathbb{R}^D, \forall i = 1, ..., I)$. The ground-truth classification label is $c$. We use $X$ to represent the input LiDAR point cloud data and $Y$ to represent all ground-truth bounding boxes in the frame. \textcolor{blue}{Here we estimate the uncertainty of location. }
%Our target here is to predict the $D \times D$ covariance matrix $\hat{\Sigma}_{i}$ for each $i$-th corner.

%We don't consider the uncertainty of classification, because \cite{feng2021review} proved that estimating classification uncertainty offers no improvement on predictive uncertainty compared with the deterministic object detector.
%\subsection{Overview of Double-M Quantification}


\subsection{Direct Modeling}
\label{sec:direct_modeling}

As introduced in the literature~\cite{meyer2020learning,he2019bounding,lakshminarayanan2017simple}, the \ac{dm} method is the classical method to estimate the aleatoric uncertainty. Here we use and modify it to estimate the aleatoric uncertainty. The main steps of~\ac{dm} are~\cite{feng2021review}:
\begin{enumerate}
    \item Select one deterministic object detector as the basic model.
    \item Set a certain probability distribution on outputs of the detector and design the corresponding loss function.
    \item Add extra regression layers at the detection head to predict the covariance.
    \item Train the modified probabilistic detector by incorporating uncertainty with the designed loss function.
\end{enumerate}

As shown in Figure~\ref{fig:main}, the basic deterministic object detector we consider here is one collaborative detector, such as one early-collaboration detector or one intermediate-collaboration detector as shown in the same figure.
% ~\ref{fig:main}. %based on the origin deterministic object detector, we use one additional header to regress the covariance matrixes and then use the predicted bounding box and covariance matrixes to describe the probability distribution of the bounding box. 

Here we assume all corners are independent, and the distribution of each corner is a multivariate Gaussian distribution:
% \begin{equation}
%     P_{\theta}(\bar{y}_i|\hat{y}_i,\hat{\Sigma}_i) = \frac{1}{\sqrt{2\pi |\hat{\Sigma}_i|}} \exp{\left(-\frac{1}{2} (y_i - \hat{y}_i)^T \hat{\Sigma}_i^{-1} (y_i - \hat{y}_i)\right)},
% \end{equation}
\begin{equation}
\nonumber
    P_{\theta}(\bar{y}_i|\hat{y}_i,\hat{\Sigma}_i) = \frac{1}{\sqrt{2\pi |\hat{\Sigma}_i|}} \exp{\left(-\frac{(\bar{y}_i - \hat{y}_i)^T \hat{\Sigma}_i^{-1} (\bar{y}_i - \hat{y}_i)}{2} \right)},
\end{equation}
where $\bar{y}_i$ is one possible vector for $i$-th corner, $\hat{\Sigma}_i$ is the $D\times D$  predicted covariance matrix for the $i$-th corner. The covariance matrix $\hat{\Sigma}_i$ is symmetric positive definite, which is implemented by the Cholesky decomposition as introduced in~\cite{kumar2020luvli}. We compare this distribution with other distributions in Section~\ref{sec:experiment} and demonstrate our selected distribution is the best.
% For one bounding box, we have $\hat{\Sigma} = \{\hat{\Sigma}_i\}_{i=1}^I$ with $\hat{y}$. \songyang{Not clear, what do you mean?}
%\hsh{In linear algebra, the Cholesky decomposition is a decomposition of a Hermitian, positive-definite matrix into the product of a lower triangular matrix and its conjugate transpose. In my opinion, it can not guarantee the positive-definite (PD). Instead, PD is a precondition to use Cholesky decomposition.}

We assume the distribution of each corner for the ground-truth bounding box as a Dirac delta function~\cite{he2019bounding}:
\begin{equation}
\nonumber
    P_G(\bar{y}_i|y_i) = \delta(\bar{y}_i - y_i).
\end{equation}

Here we define the regression loss function for the $i$-th corner as the KL-Divergence between $P_{\theta}(\bar{y}_i|\hat{y}_i,\hat{\Sigma}_i)$ and $P_G(\bar{y}_i|y_i)$~\cite{murphy2012machine}:
\begin{equation}
\begin{aligned}
    \mathcal{L}^i_{KL}(y_i, \hat{y}_i, \hat{\Sigma}_i) = & \frac{1}{2} (y_i - \hat{y}_i)^T \hat{\Sigma}_i^{-1} (y_i - \hat{y}_i) + \\ 
    &  \frac{1}{2} \log |\hat{\Sigma}_i| + \frac{\log(2\pi)}{2} - H(P_G(\bar{y}_i)),
\end{aligned} \label{eq:kl-loss}
\end{equation}
where $\frac{\log(2\pi)}{2}$ and $H(P_G(\bar{y}_i))$ could be ignored in the loss function, for thay are independent of the estimated parameters $\theta$. The first term encorages increasing the covariance of the Gaussian distribution as the predicted mean vector diverges from the ground-truth vector. The second regularization term penalizes high covariance.
% So the regression loss function is:
% \begin{equation}
%     L_{reg}(y, \hat{y}, \hat{\Sigma}) = \sum_{i=1}^E L_{KLi}(y_i, \hat{y}_i, \hat{\Sigma}_i)
% \end{equation}
We add one extra regression header to predict all covariance matrix $\hat{\Sigma}_i$ ($i \in 1,...,I$) with similar structure as the regression header for $\hat{y}_i$. 

With a given training dataset, the probabilistic direct modeling detector $f_{\theta}$ is trained to predict $\hat{Y}$, the classification possibility and the regression distribution of  all $J$ objects.
% \begin{equation}
%     f_{\theta}(X_k) = \hat{Y}_k = \{ \{\hat{p}_{jk}, \{\hat{y}_{ijk}, \hat{\Sigma}_{ijk} \}_{i=1}^I \}_{j=1}^J \}\label{eq:dm-output}
% \end{equation}
% \begin{equation}
% \begin{aligned}
%     f_{\theta}(X_m) = \hat{Y}_m = &\{ \{\hat{p}_{m1}, \{\hat{y}_{m1i}, \hat{\Sigma}_{m1i} \}_{i=1}^E \}, \\
%     &\ \ \{\hat{p}_{m2}, \{\hat{y}_{m2i}, \hat{\Sigma}_{m2i} \}_{i=1}^E \},...,\\
%     &\ \ \{\hat{p}_{mT}, \{\hat{y}_{mTi}, \hat{\Sigma}_{mTi} \}_{i=1}^E \}
%     \}
% \end{aligned}
% \end{equation}
% where $\hat{p}_{jk}$ is the predicted classification possibility for the $j$-th object in the $k$-th frame, $\hat{y}_{ijk}$ and $\hat{\Sigma}_{ijk}$ are the predicted mean vector and covariance matrix for the $i$-th corner of the $j$-th object in the $k$-th frame.
The classification loss is $\mathcal{L}_{cls}(c, \hat{p})$. The loss function of the object detection model is: 
\begin{equation}
    \mathcal{L}_{det} =  \sum_{j=1}^J(\mathcal{L}_{cls}(c_{j}, \hat{p}_{j}) + \sum_{i=1}^I \mathcal{L}^i_{KL}(y_{ij}, \hat{y}_{ij}, \hat{\Sigma}_{ij})).\label{eq:L}
\end{equation}

We train the object detection model with this loss function in~\ac{dm} method and our Double-M Quantification method.

% The model is trained by minimizing the loss function:
% \begin{equation}
%     \theta = arg \min_{\theta} L
% \end{equation}

\subsection{Double-M Quantification}
\label{sec:doubleM}
%\comment{Better name?} \songyang{direct-Modeling Moving-block bootstrap Quantification (Double-M Quantification or Two-M Quantification)}

Monte-Carlo dropout \cite{miller2018dropout} and deep ensembles \cite{lakshminarayanan2017simple} have been proposed to estimate the epistemic uncertainty. However, none of them consider the time-series features in the dataset while temporal features are important for autonomous vehicles. As a bootstrapping method on time-series data, \ac{mbb} method is able to capture the autocorrelation within the data by sampling data from the constructed data blocks \cite{lahiri1999theoretical}.
% We utilize this property of MBB  to estimate epistemic uncertainty.
We design a novel uncertainty quantification method called \ac{mdm} to estimate epistemic and aleatoric uncertainties when considering the temporal features in the dataset by combining the advantages of both the MBB  method and DM method together.

\begin{algorithm}
\caption{The training stage of Double-M Quantification }
\label{alg:mbb}
 \KwData{The training dataset $\mathbf{D}_{K} = \{ (X_{k}, Y_{k}) \}_{i=k}^{K}$ with $K$ frames, the validation dataset $\mathbf{V}_{K'} = \{ (X_{k}, Y_{k}) \}_{k=1}^{K'}$ with $K'$ frames, the block length $l$, number of bootstraps $N$, the loss function $\mathcal{L}_{det}$ in Eq~\eqref{eq:L}, the direct modeling detector $f_\theta$}
 
 \KwResult{$\hat{\theta}$,  $\Sigma_{e}$, $\Sigma_{a}$}

 % \KwInference{$\bar{\mu}_{ijk} = \hat{y}_{ijk}$, $\bar{\Sigma}_{ijk} = \Sigma_{e} + (\frac{1}{2}\Sigma_{a} + \frac{1}{2}\hat{\Sigma}_{ijk})$}
 
 $\theta_0 \leftarrow$ argmin $\mathcal{L}_{det}(\mathbf{D}_{K}, \theta)$\\
 Construct the overlapping moving-block collection $\mathbf{B} = \{\mathcal{B}_b\}_{b=1}^{K-l+1}$ from the time-series training dataset $\mathbf{D}_K$ with each block $\mathcal{B}_b = \{ (X_{b}, Y_{b}), ..., (X_{b + l - 1}, Y_{b+ l - 1}) \}, b = 1, 2, ..., K - l + 1$. \label{alg:MBB-scene} \\
% Form the time series $\{(X_{i}, Y_{i})\}_{i \geq 1}$ by periodic extension that for $i \geq 1$, $X_{i} = X_j,Y_{i} = Y_j$ if $i = mK + j$ for some integers $m \geq 0$ and $1 \leq j \leq K$\\
%  Construct a overlapping block collection from the time series data: $\mathbf{B} = \{ \mathcal{B}(i,l)\}_{i=1}^{K-l+1}$  \\
 
% $\Delta \leftarrow \{\}$\\
 \For{$n$ from $1$ to $N$}{\label{alg:MBB-boot-it-begin}
 Sample $M = \lfloor K/l \rfloor$ blocks with replacement from $\mathbf{B}$ and get a sampled dataset $\mathbf{S}_n = \{\mathcal{B}_{b_m}\}_{m=1}^{M}$ where $b_m$ are iid uniform random variables on $\{1, 2, ..., K-l+1\}$. \\ \label{alg:MBB-sample}
 Update $\theta_n \leftarrow $ argmin $\mathcal{L}_{det}(\mathbf{S}_n, \theta_{n-1})$\\ \label{alg:MBB-train}
 $f_{\theta_n}(\mathbf{V}_{K'}) = \{ \{\hat{p}_{jk}, \{\hat{y}_{ijk}, \hat{\Sigma}_{ijk}\}_{i=1}^I \}_{j=1}^J\}_{k=1}^{K'}$\\ \label{alg:MBB-test}
    % \For{$(X_k, Y_k)$\ {\rm in}\ $\mathbf{V}_{K'}$}{\label{alg:MBB-test-begin}
    % $f_{\theta}(X_{k}) = \{ \{\hat{p}_{jk}, \{\hat{y}_{ijk}, \hat{\Sigma}_{ijk}\}_{i=1}^I \}_{j=1}^J\}$\\
    % % Store $\{ \{\hat{p}_{jk}, \{\hat{y}_{ijk}, \hat{\Sigma}_{ijk}\}_{i=1}^I \}_{j=1}^J\}$ and $Y_k$ \\%into $\Delta$\\
    % }\label{alg:MBB-test-end}
  Compute the residual error $e_{ijk} = y_{ijk} - \hat{y}_{ijk}$ $\forall i\in[1,I], j\in[1,J], k\in[1,K']$ \label{alg:MBB-residual-error} \\
}\label{alg:MBB-boot-it-end}
$\hat{\theta} \leftarrow \theta_{N}$\\
Compute $\Sigma_{a}$ as the average aleatoric uncertainty of the validation dataset\\ %in $\Delta$\\
% Compute $\Sigma_{e}$ with Eq~\eqref{eq:mbb-output} %in $\Delta$\\
%Compute $\Sigma_{e}$ as the covariance of all residual error between predicted vector $\hat{y}_{ijk}$ and ground-truth vector $y_{ijk}$ ($\forall i\in[1,I], j\in[1,J], k\in[1,K]$)
Compute $\Sigma_{e}$ as the covariance of all residual errors for epistemic uncertainty \\
% \textbf{For inference:} \\ 
% \ \ \ \ $\bar{\mu}_{ijk} = \hat{y}_{ijk}$ \\ 
% \ \ \ \ $\bar{\Sigma}_{ijk} = \Sigma_{e} + (\frac{1}{2}\Sigma_{a} + \frac{1}{2}\hat{\Sigma}_{ijk})$.
\end{algorithm}

\begin{algorithm}
\caption{The inference stage of Double-M Quantification }
\label{alg:mbb-inf}
\KwData{$\Sigma_{e}$, $\Sigma_{a}$, input point cloud $X$, the direct modeling detector $f_{\hat{\theta}}$}
\KwResult{$\bar{Y}$}
$f_{\hat{\theta}}(X) = \hat{Y} = \{ \{\hat{p}_{j}, \{\hat{y}_{ij}, \hat{\Sigma}_{ij}\}_{i=1}^I \}_{j=1}^J\}$ \\
\For{j from 1 to J}{\label{alg:mbb-inf-it-start}
    \For{i from 1 to I}{
    $\bar{\Sigma}_{ij} = \Sigma_{e} + (\frac{1}{2}\Sigma_{a} + \frac{1}{2}\hat{\Sigma}_{ij})$
    }
}\label{alg:mbb-inf-it-end}
$\bar{Y} = \{ \{\hat{p}_{j}, \{\hat{y}_{ij}, \bar{\Sigma}_{ij}\}_{i=1}^I \}_{j=1}^J\}$
\end{algorithm}

%For autonomous driving datasets, there are many scenes, and each scene lasts a constant time and contains the time-series frames, which we call time-series datasets, such as nuScenes~\cite{nuscenes}, Waymo Open Dataset~\cite{sun2020scalability}, and V2X-Sim Dataset~\cite{li2022v2x}. 

We show the training stage of our proposed~\ac{mdm} method in Algorithm~\ref{alg:mbb}. We first initialize $\theta$, the prameter of a direct modeling detector and pretrain the model using the training data set. Then we construct the constant-length time-series block set $\mathbf{B}$ from the time-series training dataset $\mathbf{D}_K$ which contains $K$ frames. Notice that the block set $\mathbf{B}$ still keeps the temporal characteristics (see Line~\ref{alg:MBB-scene}) by maintaining the order of frames within the same block. Then in every training iteration, we retrain the model using a sampled dataset which contains $M$ blocks sampled with replacement and uniform random probability from the block set $\mathbf{B}$ (see Lines~\ref{alg:MBB-sample}--\ref{alg:MBB-train}). The sampled dataset still contains about $K$ frames since $M=\lfloor K/l \rfloor$ . The floor function $\lfloor \cdot \rfloor$ is to make sure $M$ is an integer. As the final step in each training iteration $n$, we test the retained model $f_{\theta_n}$ on the validation dataset $\mathbf{V}_{K'}$ (see Line~\ref{alg:MBB-test}) and compute the residual vector, i.e. the difference between the predicted mean vector $\hat{y}_{ijk}$ and the ground-truth vector $y_{ijk}$, $\forall i\in[1,I], j\in[1,J], k\in[1,K']$ (see Line~\ref{alg:MBB-residual-error}). After $N$ iterations, we get the final model parameters $\theta_N$ as $\hat{\theta}$ so that our~\ac{mdm} method could predict the uncertainty by model $f_{\hat{\theta}}$. Other than the final trained model, we estimate both the aleatoric and epistemic uncertainties by using the residuals and predicted covariance matrics of the validation dataset. We first estimate the aleatoric uncertainty by computing $\Sigma_{a}$, the mean of all the predicted covariance matrices. To estimate the epistemic uncertainty, we then compute the covariance matrix of all residual vectors, which is denoted by $\Sigma_{e}$. On the one hand, our Dourble-M Quantification method provides the bagging aleatoric uncertainty estimates through the aggrgation over multiple models from the $N$ iterations. On the other hand, it approximates the distribution of errors from the residuals so that we can quantify the epistemic uncertainties.
% \begin{equation}
% \begin{aligned}
%      r_{ijk} = &y_{ijk} - \hat{y}_{ijk} , \forall i\in[1,I], j\in[1,J], k\in[1,K]\\
%     \Sigma_{eij} = &Cov(R) \comment{Need to modify}
% \end{aligned}\label{eq:mbb-output}
% \end{equation}
% where $\mathbb{E}(*)$ is the expected value.

%During inference, for the $i$th corner of the $j$th bounding box, we use $\hat{y}_{ij}$ as the mean of the multivariate Gaussian distribution. We combine the $\Sigma_{e}$, $\Sigma_{a}$ and predicted covariance matrix $\hat{\Sigma}_{ij}$ from the extra regression header as the covariance $\bar{\Sigma}_{ij}$ of the distribution:
 The Inference stage of our~\ac{mdm} method is shown in Algorithm~\ref{alg:mbb-inf}. For the $i$th corner of the $j$th bounding box, we use $\hat{y}_{ij}$ as the mean of the multivariate Gaussian distribution. we estimate the covariance matrix $\bar{\Sigma}_{ij}$ by using (i) the predicted covariance matrix $\hat{\Sigma}_{ij}$ from the extra regression header and (ii) the estimated aleatoric and epistemic uncertainties $\Sigma_{e}$, $\Sigma_{a}$ obtained from the training stage of the proposed Double-M Quantification algorithm.  $\bar{\Sigma}_{ij}$ is calculated as the following:
\begin{equation}
\begin{aligned}
    % \bar{\mu}_{ij} = & \hat{y}_{ijk}, \\
    \bar{\Sigma}_{ij} = \Sigma_{e} + (\frac{1}{2}\Sigma_{a} + \frac{1}{2}\hat{\Sigma}_{ij}).
\end{aligned}\label{eq:cov-comb-output}
\end{equation}

% \comment{Theory Explanation @Sihong}

% \textbf{\ac{mbb} method without~\ac{dm}:} \comment{move to experiment}
% For the $m$th frame in $V_{K}$, the outputs of the object detection model $f_{\theta}$ are:
% \begin{equation}
%     f_{\theta}(X_{m}) = \{ \{\hat{p}_{mt}, \{\hat{y}_{mti}\}_{i=1}^E \}\}_{t=1}^T
%     \}
% \end{equation}

% We use the covariance matrix $\Sigma_{e}$ of the residual error between predicted vector $\hat{y}_{mti}$ and ground-truth vector $y_{mti}$ ($\forall m\in[1,K], t\in[1,T], i\in[1,4]$) as the covariance matrix of epistemic uncertainty for all data.

% \begin{equation}
% \begin{aligned}
%      r_{mti} = &y_{mti} - \hat{y}_{mti} , \forall m\in[1,K], t\in[1,T], i\in[1,4]\\
%     \Sigma_{e} = &\mathbb{E}((r_{mti} - \mathbb{E}(r_{mti}))(r_{mti} - \mathbb{E}(r_{mti}))^T)
% \end{aligned}\label{eq:mbb-output}
% \end{equation}
% where $\mathbb{E}(*)$ is the expected value. During inference, we use $\Sigma_{e}$ as the estimated covariance matrix for all corners.

% \textbf{\ac{mbb} method with~\ac{dm}:}
% For the $m$th frame in $V_{K}$, the outputs of the object detection model $f_{\theta}$ are shown as Eq~\ref{eq:dm-output}.

% Here we use the $\Sigma_{e}$ as Eq~\ref{eq:mbb-output} and the mean of all predicted covariance matrixes $\hat{\Sigma}_{mti}$ which is called $\Sigma_{a}$ and useful for estimating the aleatoric uncertainty.

% During inference, we combine the $\Sigma_{e}$, $\Sigma_{a}$ and predicted covariance matrix $\hat{\Sigma}_{mti}$ from the additional regression header as the estimated covariance matrix for the $i$th corner of the $t$th bounding box in the $m$th frame:
% \begin{equation}
%     \bar{\Sigma}_{mti} = w\Sigma_{e} + (1-w)(\frac{1}{2}\Sigma_{a} + \frac{1}{2}\hat{\Sigma}_{mti})\label{eq:cov-comb-output}
% \end{equation}
% where $w$ is one hyperparameter trading off the epistemic uncertainty and the aleatoric uncertainty.

==> old_introduction.tex <==
\section{introduction}
\label{sec:intro}
\comment{1. object detection, emp the important
2. uncertainty challenge (songyang)
3. uncertainty quantificatiom, only put review paper and good paper
4. introduce coll object detection..
5. Exist methods on sinlge-agent object detection cannot be used on collaborate object detection directly (important). For example, dropout cannot be used on intermediate fusion... 6. introduce our work and contribution
}
\songyang{Autonomous vehicles may have uncertain object detection due to out-of-distribution objects, sensor measurement noise, poor weather, or illumination conditions~\cite{liu2021robust,kothandaraman2021ss,feng2021review}. Even a slightly false detection result can lead the autonomous vehicle's driving policy to a completely different action~\cite{huang2017adversarial,lin2017tactics}. For example, a miss-detected paint on the road surface can confuse an autonomous vehicle's lane-following policy and cause potential accidents~\cite{kurakin2016adversarial}. Therefore, it is crucial to quantify the uncertainty of object detection for safety-critical applications, like autonomous vehicles.}

Object detection aims to classify and localize surrounding traffic objects from sensor data frame by frame~\cite{qian20223d}. In recent years, deep learning has been the mainstream approach to object detection. And many uncertainty quantification methods have been proposed for deep learning object detection~\cite{meyer2020learning,he2019bounding,miller2018dropout,lakshminarayanan2017simple, hall2020probabilistic,harakeh2021estimating,chiu2021probabilistic,gustafsson2020evaluating,miller2019evaluating,ali2020bayesod,meyer2019lasernet,lee2022trust}. In deep learning, uncertainty can be decomposed into the aleatoric uncertainty and the epistemic uncertainty~\cite{feng2021review, hullermeier2021aleatoric,kendall2017uncertainties}. Aleatoric uncertainty (or data uncertainty) represents the inherent measure noises from the sensor. 
For example, detecting objects only with RGB cameras at night trends to produce high aleatoric uncertainty. The aleatoric uncertainty is mainly estimated by the Direct modeling~\cite{meyer2020learning,he2019bounding}. 
Epistemic uncertainty (or model uncertainty) reflects the degree of uncertainty that a model describes an observed dataset with its parameters. For example, an out-of-distribution object, such as a motorized tricycle which is only seen in Asian cities, tends to be detected with high epistemic uncertainty.  Monte-Carlo Dropout~\cite{gal2017concrete,miller2018dropout} and Deep Ensembles~\cite{lakshminarayanan2017simple} are usually used to capture the epistemic uncertainty. 
However, none of these methods has been used to estimate the uncertainty of collaborative 3D object detection.

\comment{Multi-agent collaborative detection has been proposed to leverage the viewpoints from other agents in order to upgrade the detection with individual viewpoint~\cite{li2022v2x}. Recent research has shown the effectiveness of early, late, and intermediate collaboration, which respectively transmit raw data, output bounding boxes, and intermediate features~\cite{li2021learning,Chen2019CooperCP,arnold2020cooperative}.  }

In this paper, we propose a novel uncertainty quantification method Direct Moving Block Bootstrap Modeling, which is based on Moving Block Bootstrap~\cite{lahiri1999theoretical} and Direct Modeling. Our method could estimate the aleatoric uncetrainty and the epistemic uncertainty with one inference. Then we apply our method on collaborative 3D object detection, which is the first one to do it. Here we only estimate the uncertainty of location, because \cite{feng2021review} proved that estimating classification uncertainty offers no improvement on predictive uncertainty compared with the deterministic object detector. With the probabilistic collaborative object detectiors, we could construct the safety range for each detected object as shown in Figure~\cite{fig:vis}, which would help the later module in the autonomous driving, such as trajectory prediction~\cite{boris2022propagating} and planning\comment{find reference}.  Experiments on the comprehensive collaborative perception dataset~\cite{li2022v2x} showed that our uncertainty quantification method could estimate the uncertainty better without accuracy overhead. For collaborative Object detection, experiments showed that collaboration between autonomous vehicles could not only improve the accuracy of detection but also reduce the uncertainty. The  code for our method will be available on GitHub upon publication.

The main contributions of this work are as follows:
\begin{enumerate}
    \item To our knowledge, this is the first work to estimate the uncertainty of collaborative 3D object detection. We showed that sharing information between autonomous vehicle could reduce uncertainty.
    \item We propose an uncertainty quantification method Direct Moving Block Bootstrap Modeling which could estimate uncertainty better without accuracy overhead.
\end{enumerate}

The rest of this paper is organized as follows. Section~\ref{sec:relatedwork} discussed the related works. Section~\ref{sec:collab} introduce the collaborative 3D object detection in detail. Section~\ref{sec:approach} presents our uncertainty quantification method. Section~\ref{sec:experiment} shows the experimental results. Finally, Section~\ref{sec:conclusion} concludes the paper.

==> old_relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

\textbf{Collaborative 3D Object Detection.} Collaborative object detection, in which multiple agents collectively perceive a scene via communication, is able to address several dilemmas in individual object detection~\cite{li2022v2x}. Compared to individual detection, multi-agent collaboration introduces more viewpoints to solve the long-range data sparsity stemming from the restricted sensing capability and to mitigate the influence of severe occlusion in dense traffic scenarios. The pioneer collaborative detectors employ early collaboration which shares raw data~\cite{Chen2019CooperCP} or late collaboration which shares output bounding boxes~\cite{arnold2020cooperative}. To further improve the performance-bandwidth trade-off, recent research proposes intermediate collaboration which shares intermediate feature representations from a neural network. Various intermediate collaboration strategies have been developed such as neural message passing~\cite{wang2020v2vnet}, knowledge distillation~\cite{li2021learning}, and attention~\cite{xu2022v2x}. Most works focus on improving the performance of collaborative detection, yet few works have investigated uncertainty quantification in collaborative object detection. \songyang{However, the above works only focus on improving the performance of collaborative detection without considering the uncertainties of the detection results. To the best of our knowledge, we make the first attempt to quantify uncertainty in collaborative object detection.}

\textbf{Uncertainty Quantification on Object Detection.} 
\comment{
1. unrelated part, dropout and ensembles
2. The closest works for ours are direct modeling and bootstrap (estimate the tempor-based dataset).
}
\songyang{Though Direct Modeling (DM) has been widely used to quantify aleatoric uncertainty for single-view autonomous vehicles, how to use DM to quantify uncertainties in multi-view collaborative detection is still a challenge.} Many uncertainty quantification methods for object detection have been proposed. For the aleatoric uncertainty, Direct Modeling (DM) is the usual method. It assumes a certain probability distribution on the outputs, uses network layers to directly predict parameters of the distribution, and uses the Kullback-Leibler divergence between the predictive probability distribution and the groud-truth distribution as the loss function for training. The work~\cite{he2019bounding} proposes the DM method for 2D image object detection, which assumes the distribution of each bounding box variable is single variate Gaussian distribution and introduces one additional layer to estimate the variance of the bounding box. \cite{meyer2019lasernet,meyer2020learning} apply the Direct Modeling method to 3D object detection with independent univariate Laplace distribution assumption. In our work, we also use the DM method to estimate the aleatoric uncertainty of collaborative 3D object detection with a multivariate Gaussian distribution assumption.

For epistemic uncertainty, Monte-Carlo Dropout and Deep Ensembles are common methods. The MC Dropout method utilizes the dropout-based neural network training to perform approximate inference in Bayesian Neural Networks. \cite{miller2018dropout} uses MC Dropout on 2D image object detection to improve accuracy. Deep Ensembles estimate probability distribution by an ensemble of networks with the same architecture and different parameters after training~\cite{lyu2020probabilistic, lakshminarayanan2017simple,ovadia2019can}. Both of them require multiple runs for inference which makes them infeasible for real-time critical tasks with high computational costs. What is more, they don't consider the time series in the dataset which is one characteristic of the autonomous driving dataset. However, our uncertainty quantification method could overcome these problems by using Moving Block Bootstrap.

Many works estimate both uncertainties by using some of these methods. \cite{kendall2017uncertainties,feng2019leveraging,feng2018towards} estimates the aleatoric and epistemic uncertainties in 3D object detection with DM and MC dropout respectively. All the above works only focus on single-agent object detection. However, our work estimates both uncertainties for collaborative 3D object detection.
